A Norm-Minimization Algorithm for Solving the Cold-Start Problem with XNAV

An algorithm is presented for solving the cold-start problem using observations of X-ray pulsars. Using a norm-minimization-based approach, the algorithm extends Lohan's banded-error intersection model to 3-dimensional space while reducing compute time by an order of magnitude. Higher-fidelity X-ray pulsar signal models, including the parallax effect, Shapiro delay, time dilation, and higher-order pulsar timing models, are considered. The feasibility of solving the cold-start problem using X-ray pulsar navigation is revisited with the improved models and prior knowledge requirements are discussed. Monte Carlo simulations are used to establish upper bounds on uncertainty and determine the accuracy of the algorithm. Results indicate that it is necessary to account for the parallax effect, time dilation, and higher-order pulsar timing models in order to successfully determine the position of the spacecraft in a cold-start scenario. The algorithm can uniquely identify a candidate spacecraft position within a 10 AU $\times$ 10 AU $\times$ 0.01 AU spheroid domain by observing eight to nine pulsars. The median position error of the algorithm is on the order of 15 km. Prior knowledge of spacecraft position is technically required, but only to an accuracy of 100 AU, making it practically unnecessary for navigation within the Solar System. Results further indicate that choosing lower-frequency pulsars increases the maximum domain size but also increases position error.

==> 99_future.tex <==
%!TEX root = _main.tex
\section{Conclusion and Expected Work for Final Publication}
\label{sec:future}

A norm-minimization-based XNAV algorithm was proposed to solve the cold-start problem. The Shapiro delay, parallax effect, Einstein delay, and pulsar frequency variations were incorporated into both the simulation and the solver, in addition to the first order Doppler delay considered by existing studies. It was found that the Einstein delay must be estimated to within 0.1 ms for reliable convergence of the algorithm. It was also found that the other effects listed above constrain the reference point for pulsar timing models to be within 2 AU of the true position for reliable convergence. 

For the final publication, additional simulation results of the impact of the Shapiro delay, parallax effect, and pulsar frequency variation will be added to the analysis. The impact of measurement quality in the form of phase uncertainty, as well as pulsar selection, will also be analyzed. 

%Primarily, more Monte Carlo simulations must be performed to assess the convergence probability and accuracy of the algorithm under various conditions. 
%
%The phase measurement uncertainty can be affected by the sensor quality and/or the total duration for pulsar observations. There may be an upper bound for phase uncertainty, because if the phase uncertainty is too large, too many intersections will be created, resulting in multiple candidate points that cannot be resolved. 
%
%The number of pulsars observed also affects how candidate points are narrowed down. Fewer pulsars means fewer wavefronts to intersect, leading to a higher chance for finding multiple candidate points. On the other hand, more pulsars may cause the algorithm to eliminate the true solution. 
%
%Finally, existing Monte Carlo test results will be updated, especially Figure~\ref{fig:conv_models} as described in the corresponding paragraphs.
